EHRCon: Dataset for Checking Consistency between Unstructured Notes and Structured Tables in Electronic Health Records

Electronic Health Records (EHRs) are integral for storing comprehensive patient medical records, combining structured data (e.g., medications) with detailed clinical notes (e.g., physician notes). These elements are essential for straightforward data retrieval and provide deep, contextual insights into patient care. However, they often suffer from discrepancies due to unintuitive EHR system designs and human errors, posing serious risks to patient safety. To address this, we developed EHRCon, a new dataset and task specifically designed to ensure data consistency between structured tables and unstructured notes in EHRs. EHRCon was crafted in collaboration with healthcare professionals using the MIMIC-III EHR dataset, and includes manual annotations of 4,101 entities across 105 clinical notes checked against database entries for consistency. EHRCon has two versions, one using the original MIMIC-III schema, and another using the OMOP CDM schema, in order to increase its applicability and generalizability. Furthermore, leveraging the capabilities of large language models, we introduce CheckEHR, a novel framework for verifying the consistency between clinical notes and database tables. CheckEHR utilizes an eight-stage process and shows promising results in both few-shot and zero-shot settings. The code is available at https://github.com/dustn1259/EHRCon.

==> algorithm/segmentation.tex <==
\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% \begin{multicols}{2}
% \noindent
% \begin{minipage}[H]{0.35\textwidth}

% \end{minipage}
% \begin{minipage}[H]{0.6\textwidth}
% \begin{algorithm}[H]
% \caption{Note Segmentation Process}
% \label{alg:findmax}
% \begin{algorithmic}[1]
% \vspace{1em}
% \REQUIRE Clinical Note $P$, Maximum Length of Subtext $l$
% \ENSURE Set of Subtexts $\mathcal{T}$
% \STATE $\mathcal{T} \leftarrow \emptyset, i \leftarrow 0, P_i \leftarrow P$
% \WHILE{$TokenLen(P_i)$ $ > l$}
%     \STATE $P^f_i, P^b_i \leftarrow DivideByLen(P_i, l)$
%     \STATE $P^f_{i, 0}, P^f_{i, 1}, P^f_{i, 2} \leftarrow DivideByLLM(P^f_i)$
%     \STATE $\mathcal{T} \leftarrow \mathcal{T} \cup \{P^f_{i, 0}, P^f_{i, 1}\}$
%     \STATE $P_{i+1} \leftarrow MergeText(P^f_{i, 2}, P^b_i)$
%     \STATE $i \leftarrow i+1$    
% \ENDWHILE
% \STATE $\mathcal{T} \leftarrow \mathcal{T} \cup \{P_{i}\}$
% \STATE $\mathcal{T} \leftarrow MakeIntersection(\mathcal{T})$
% \RETURN $\mathcal{T}$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \end{multicols}




==> app_fig/about_nursing_other.tex <==
\begin{tcolorbox}[
    colback=white,
    fonttitle=\bfseries,
    coltitle=white,
]
Family Meeting Note\\
Family meeting held with both Social Worker, nurse and myself. \\The discharge for the 98/02/02 set, scheduled for might not proceed as s potentially unprepared. Pediatrician identified. \\Location A desire circumcision prior to discharge. 
\label{nursing_other}
\end{tcolorbox}
%To protect patient privacy, all values in the example data mentioned in the paper have been replaced with fictional values, and some sentences have been paraphrased. 

==> app_fig/col_map_instruct.tex <==
\begin{tcolorbox}[
    colback=white,
]
\{`value': \{`labevents': `valuenum', `chartevents': `valuenum', `inputevents\_cv': `amount',\\
`inputevents\_cv': `rate', 'outputevents': `valuenum', `prescriptions': `dose\_val\_rx',\\
`inputevents\_mv': `rate', 'inputevents\_mv': `amount'\},\\


\{`unit': \{`chartevents': `valueuom', `inputevents\_cv': `amountuom', `inputevents\_cv':`rateuom',`inputevents\_mv': `rateuom',`inputevents\_mv': `amoutuom
`labevents': `valueuom', `outputevents': `valueuom', `prescriptions': `dose\_unit\_rx'\}\}\\


\{'time' : \{'chartevents':'charttime','labevents':'charttime','outputevents':'charttime',\\
'inputevents\_cv':'charttime', 'microbiologyevents':'charttime', 'inputevents\_mv':'starttime','inputevents\_mv':'endtime',\\
'prescriptions':'startdate', 'prescriptions': 'enddate'\}\\

\{'organism':\{'microbiologyevents':'org\_name'\}, \\

\{'specimen': \{'microbiologyevents':'spec\_type\_desc'\} \}]\\
\end{tcolorbox}

==> contents/ablation.tex <==
To conduct an in-depth analysis of our framework's bottlenecks, we performed additional analysis on 25\% of the entire test set. We provided the ground truth for stages we considered crucial, and conducted experiments with a total of four different settings. We found that the table selection process yielded the least performance improvement, indicating that it is the least significant bottleneck. This suggests that the complexity of this task is lower compared to other stages. On the other hand, removing the Pseudo Table Creation step resulted in the most significant performance improvement. This indicates that the LLM still has limitations in converting free-text into a structured format.

==> tab/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% \begin{wraptable}{r}{0.6\columnwidth}
% % \begin{table}[]
% \vspace{-5mm}
% \caption{Ablation study for each stage.}
% \resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{c|l|cc}
% \Xhline{0.3mm}
% \textbf{Models} & \multicolumn{1}{c|}{\textbf{Experiment Setting}} & \textbf{Rec} & \textbf{Prec} \\ \hline
% \multirow{5}{*}{\textbf{ChatGPT-3.5}} & CheckEHR & 65.45 & 54.61 \\
%  & - NER &  71.81 & 76.26 \\
%  & - NER$'$ & 76.11 & 77.7 \\
%  & - (Table Identification + Time Filtering) & 82.49 & 78.99 \\
%  & - Pseudo Table Creation & 92.83 & 94.93 \\ \Xhline{0.3mm}
% \end{tabular}%
% }\label{chatgptablation}
% % \end{table}
% \vspace{-5mm}
% \end{wraptable}

==> tab/ner_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccclcclcclcc}
\hline
\multirow{2}{*}{\textbf{Settings}} & \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Nursing}} & \textbf{} & \multicolumn{2}{c}{\textbf{Discharge}} & \textbf{} & \multicolumn{2}{c}{\textbf{Physician}} & \textbf{} & \multicolumn{2}{c}{\textbf{Total}} \\ \cline{3-4} \cline{6-7} \cline{9-10} \cline{12-13} 
 &  & Rec & Prec &  & Rec & Prec &  & Rec & Prec &  & Rec & Prec \\ \hline
\multirow{3}{*}{Few-Shot} & TULU-2 & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\
 & Mixtral & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\
 & Llama-3 & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\ \hline
\multirow{3}{*}{Zero-Shot} & TULU-2 & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\
 & Mixtral & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\
 & Llama & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 &  & 0.0 & 0.0 \\ \hline
\end{tabular}%
}
\end{table}

==> tab/omopzero_item.tex <==
\begin{table}[h]
\centering
\begin{minipage}{0.57\textwidth}
\caption{Results of experiments for component analysis conducted by matching entities with items in the database. 
In our experiment, we bypassed the named entity recognition (NER) step and directly provided gold entities.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}-Additional \\ Manual Annotation\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}+Additional \\ Manual Annotation\end{tabular}}} \\ \cline{2-5} 
 & \textbf{Rec} & \textbf{Prec} & \textbf{Rec} & \textbf{Prec} \\ \hline
\textbf{Tulu2} & 61.56 & 65.07 & 61.86 & 66.35 \\
\textbf{Mixtral} & 65.07 & 70.21 & 66.35 & 70.51 \\
\textbf{Llama3} & 59.23 & 56.16 & 60.33 & 64.67 \\
\textbf{GPT-3.5 (0613)} & 71.81 & 76.25 & 76.11 & 77.70 \\ \hline
\end{tabular}%
}\label{item_search_ab}
\end{minipage}
\hfill
\begin{minipage}{0.38\textwidth}
\caption{OMOP zero-shot results.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc}
\hline
Model & \textbf{Rec} & \textbf{prec} \\ \hline
\textbf{Tulu2} &  &  \\
\textbf{Mixtral} &  &  \\
\textbf{Llama-3} &  &  \\ \hline
\end{tabular}%
}
\end{minipage}
\end{table}

==> tab/prompts/named_entity_recognition_prompt_zero.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|}
\hline
\multicolumn{1}{|c|}{\textbf{description2}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Your task is to analyze a clinical note and divide it into three sections based on thematic or semantic coherence.\\ Each section should center around a unique theme or idea, providing a cohesive view of the content. \\ \\
Please follow these guidelines: \\ 
Guidelines 1) Thematic or Semantic Unity:  Group content based on clear thematic or semantic relationships, ensuring \\that each section covers a distinct aspect related to the overall topic. Everything within a section should be related and\\contribute to a unified understanding of that theme. \\\\Guidelines 2) Equal Length and Comprehensive Coverage: Strive for a balance in the length of each section, \\but also consider the depth and breadth of the content. The division should reflect an equitable distribution of information, \\without sacrificing the completeness of any thematic area. This balance is essential to ensure no single section is \\overwhelmingly long or short compared to the others.\\\\Guidelines 3) Integrity of Sections: Pay close attention to the natural divisions within the text, such as headings or topic \\changes (e.g., "History of Present Illness," "Past Medical History," "Medications"). Ensure that these content blocks are \\not fragmented across sections. A section should encompass complete thoughts or topics to preserve the logical flow \\and coherence of information. \\\\
Guidelines 5) Output format must be [section1: (start\_line\_number-end\_line\_number), section2: (start\_line\_number-\\end\_line\_number), section3: (start\_line\_number-end\_line\_number)].\\\\Guidelines 6) Precise Output Format and Continuous Line Coverage: The start line number in section 1 should match\\ the start number of the given text and the end line number in section 3 should match the last line number of the given text.\\ Ensure sections are contiguous; the end of one section immediately precedes the start of the next, with no gaps or overlaps.\\\\
To prevent sentences from being split between sections, carefully review the end of each proposed section. If a \\sentence starts in one  section and continues into the next, adjust the section boundaries accordingly to ensure sentence \\integrity. This may require you to slightly rebalance the length of the sections to accommodate full sentences while \\still adhering to the guidelines for thematic unity, comprehensive coverage, and equal length.\\\\

Example 1)\\\\
Clinical Note: \\ 
"44 On transfer, vitals were T 93.1, HR 67 , BP 1120/76, RR
35 20, O2sat 99.9\% on 2LNC. \\

...\\\\

58 Past Medical History:\\
59 1. CARDIAC RISK FACTORS: +Hypertension, +HLD\\
60 2. CARDIAC HISTORY:"\\
output format must be [section1: (start\_number\_of\_the\_given\_text-end\_line\_number), \\section2: (end\_line\_number-end\_line\_number), section3: (end\_line\_number-last\_number\_of\_given\_text)]\\
Output: [section1: 44-50, section2: 50-57, section3: 58-60]\\\\


....\\\\

Your task)\\
Clinical Note: \\ \textless{}\textless{}\textless{}\textless{}CLINICAL\_NOTE\textgreater{}\textgreater{}\textgreater{}\textgreater{}\\\\
output: [section1: (start\_number\_of\_the\_given\_text-end\_line\_number), section2: (end\_line\_number-end\_line\_number),\\ section3: (end\_line\_number-last\_number\_of\_given\_text)]\\


\end{tabular} \\




\hline


\end{tabular}%
}
\caption{Zero Shot Prompt for Note Segmentation2
}
\end{table*}

==> tab/prompts/note_segmentation_zero.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|}
\hline
\multicolumn{1}{|c|}{\textbf{description}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Your task is to analyze a clinical note and divide it into three sections based on thematic or semantic coherence.\\ Each section should center around a unique theme or idea, providing a cohesive view of the content. \\ \\
Please follow these guidelines: \\ 
Guidelines 1) Thematic or Semantic Unity:  Group content based on clear thematic or semantic relationships, ensuring \\that each section covers a distinct aspect related to the overall topic. Everything within a section should be related and\\contribute to a unified understanding of that theme. \\\\Guidelines 2) Equal Length and Comprehensive Coverage: Strive for a balance in the length of each section, \\but also consider the depth and breadth of the content. The division should reflect an equitable distribution of information, \\without sacrificing the completeness of any thematic area. This balance is essential to ensure no single section is \\overwhelmingly long or short compared to the others.\\\\Guidelines 3) Integrity of Sections: Pay close attention to the natural divisions within the text, such as headings or topic \\changes (e.g., "History of Present Illness," "Past Medical History," "Medications"). Ensure that these content blocks are \\not fragmented across sections. A section should encompass complete thoughts or topics to preserve the logical flow \\and coherence of information. \\\\
Guidelines 5) Output format must be [section1: (start\_line\_number-end\_line\_number), section2: (start\_line\_number-\\end\_line\_number), section3: (start\_line\_number-end\_line\_number)].\\\\Guidelines 6) Precise Output Format and Continuous Line Coverage: The start line number in section 1 should match\\ the start number of the given text and the end line number in section 3 should match the last line number of the given text.\\ Ensure sections are contiguous; the end of one section immediately precedes the start of the next, with no gaps or overlaps.\\\\
To prevent sentences from being split between sections, carefully review the end of each proposed section. If a \\sentence starts in one  section and continues into the next, adjust the section boundaries accordingly to ensure sentence \\integrity. This may require you to slightly rebalance the length of the sections to accommodate full sentences while \\still adhering to the guidelines for thematic unity, comprehensive coverage, and equal length.\\\\

Example 1)\\\\
Clinical Note: \\ 
"44 On transfer, vitals were T 93.1, HR 67 , BP 1120/76, RR
35 20, O2sat 99.9\% on 2LNC. \\

...\\\\

58 Past Medical History:\\
59 1. CARDIAC RISK FACTORS: +Hypertension, +HLD\\
60 2. CARDIAC HISTORY:"\\
output format must be [section1: (start\_number\_of\_the\_given\_text-end\_line\_number), \\section2: (end\_line\_number-end\_line\_number), section3: (end\_line\_number-last\_number\_of\_given\_text)]\\
Output: [section1: 44-50, section2: 50-57, section3: 58-60]\\\\


....\\\\

Your task)\\
Clinical Note: \\ \textless{}\textless{}\textless{}\textless{}CLINICAL\_NOTE\textgreater{}\textgreater{}\textgreater{}\textgreater{}\\\\
output: [section1: (start\_number\_of\_the\_given\_text-end\_line\_number), section2: (end\_line\_number-end\_line\_number),\\ section3: (end\_line\_number-last\_number\_of\_given\_text)]\\


\end{tabular} \\




\hline


\end{tabular}%
}
\caption{Zero Shot Prompt for Note Segmentation
\label{tab:zero_shot_note_segmentation}
}
\end{table*}

==> tab/zero_omop_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{zeroshot omop result}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccclcclcclcc}
\hline
\multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Discharge Summary}} & \textbf{} & \multicolumn{2}{c}{\textbf{Physician Note}} & \textbf{} & \multicolumn{2}{c}{\textbf{Nursing Note}} & \textbf{} & \multicolumn{2}{c}{\textbf{Total}} \\ \cline{3-4} \cline{6-7} \cline{9-10} \cline{12-13} 
                                  &                                  & Rec                   & Prec                   &           & Rec                  & Prec                 &           & Rec                 & Prec                &           & Rec                & Prec          \\ \hline
\multirow{3}{*}{Zero}             & Tulu2                            &                       &                        &           &                      &                      &           &                     &                     &           &                    &               \\
                                  & Mixtral                          & -                     & -                      &           & -                    & -                    &           & -                   & -                   &           & -                  & -             \\
                                  & Llama-3                          &                       &                        &           &                      &                      &           &                     &                     &           & \textbf{}          &               \\ \hline
\end{tabular}
}
\end{table}
